Community Detection Across Emerging Quantum Architectures

One of the roadmap plans for quantum computers is an integration within HPC ecosystems assigning them a role of accelerators for a variety of computationally hard tasks. However, in the near term, quantum hardware will be in a constant state of change. Heading towards solving real-world problems, we advocate development of portable, architecture-agnostic hybrid quantum-classical frameworks and demonstrate one for the community detection problem evaluated using quantum annealing and gate-based universal quantum computation paradigms.

==> results.tex <==
Refinement heuristics
\begin{enumerate}
\item Top Gain (TP)
\item Spectral Ordering (SP)
\item Reverse Cuthill-McKee Ordering (RCM)
\end{enumerate}
\begin{table}[hp]
\caption{TG (standalone, stopping criteria is same subset)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
    arenas-jazz& 0.2897 & 0.3082& 0.3206 & 0.0103& 5.0&7.0667& 10.0& 1.0625
\\ \hline
arenas-meta &0.2339& 0.2721& 0.3158& 0.0228& 10.0& 15.1& 31.0& 4.3844
\\ \hline
brunson &0.3322& 0.4098& 0.4310& 0.0234& 3.0& 4.0667& 5.0& 0.3590 \\ \hline
contact &0.0755& 0.0896& 0.1051& 0.0079& 6.0& 9.4667& 17.0& 2.247  \\ \hline
moreno\_oz &0.239& 0.3099& 0.3388& 0.0259& 7.0& 9.9& 16.0& 2.3144
 \\ \hline
 sociopatterns\_infectious&0.3612& 0.4137& 0.4633& 0.028& 9.0& 12.9333& 18.0& 2.1592\\
    \hline
  \end{tabular}
\end{table}

\begin{table}[hp]
\caption{TG + SP (standalone, stopping criteria is 5 iterations of no improvement)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
    arenas-jazz& 0.2907& 0.308& 0.3206& 0.0087& 14.0& 17.7667& 22.0& 2.1242
\\ \hline
arenas-meta &0.2369& 0.2771& 0.3168& 0.024& 33.0& 46.8333& 72.0& 8.9743
\\ \hline
brunson & 0.3836& 0.4215& 0.431& 0.0147& 7.0& 9.3& 12.0& 1.0376
\\ \hline
contact &  0.0805& 0.0966& 0.107& 0.0074& 20.0& 27.7& 49.0& 6.149
\\ \hline
moreno\_oz &0.2692& 0.3243& 0.3388& 0.0211& 15.0& 27.2667& 54.0& 8.9664
 \\ \hline
 sociopatterns\_infectious&0.3996& 0.4415& 0.4633& 0.0186& 25.0& 31.7& 36.0& 2.571
\\
    \hline
  \end{tabular}
  \end{table}
  
  \begin{table}[hp]
\caption{TG + SP + threshold (30 different seeds, main implementation, , stopping criteria is 3 iterations of no improvement)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
arenas\_jazz & 0.2902 & 0.309 & 0.3206 & 0.0087 & 14.0 & 20.1333 & 26.0 & 2.617\\ \hline
arenas\_meta & 0.2451 & 0.2778 & 0.3143 & 0.0212 & 34.0 & 43.3333 & 66.0 & 7.7775\\ \hline
brunson & 0.3319 & 0.4149 & 0.4309 & 0.0227 & 13.0 & 15.2 & 20.0 & 1.5362\\ \hline
contact & 0.0772 & 0.0954 & 0.1102 & 0.0092 & 20.0 & 28.0 & 53.0 & 6.1319\\ \hline
moreno\_oz\_oz & 0.266 & 0.3196 & 0.3388 & 0.0253 & 17.0 & 25.2333 & 44.0 & 6.766\\ \hline
sociopatterns\_infectious & 0.3923 & 0.4423 & 0.4633 & 0.0191 & 27.0 & 32.4667 & 39.0 & 3.2221\\ \hline

  \end{tabular}
  \label{tab:TGSPthresholdmainimplementation}
  \end{table}
  
For Table \ref{tab:TGSPthresholdmainimplementation}:
\scriptsize
\begin{lstlisting}
for g in /zfs/safrolab/users/dwave_vs_qaoa/graphs/*/out.*
    do
        for seed in 1070 8173 3509 8887 1314 4506 5219 3765 1420 7778 3734 6509 1266 5063 6496 4622 7018 6052 8932 8215 1254 400 3260 5999 1331 8073 7357 2928 7208 3874
            do python -W ignore single_level_refinement.py --graph $g --method optimal --iter-size 25 --stopping-criteria 3 --seed $seed --subset spectral
    done
done
\end{lstlisting}
  
  \begin{table}[hp]
\caption{TG + SP + same part (standalone)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
    arenas-jazz& 0.2973& 0.306& 0.3206& 0.0087& 6.0& 11.2333& 17.0& 3.2423

\\ \hline
arenas-meta &0.2428& 0.2954& 0.3168& 0.0188& 27.0& 36.6333& 56.0& 6.8141

\\ \hline
brunson & 0.3068& 0.4261& 0.431& 0.0226& 4.0& 5.8& 7.0& 0.7483

\\ \hline
contact &  0.0748& 0.1018& 0.1106& 0.0098& 19.0& 24.9& 38.0& 5.3935

\\ \hline
moreno\_oz &0.3269& 0.338& 0.3388& 0.0026& 11.0& 13.1667& 19.0& 1.7904

 \\ \hline
 sociopatterns\_infectious&0.4192& 0.4524& 0.4633& 0.0157& 10.0& 13.4333& 19.0& 2.4039

\\
    \hline
  \end{tabular}
\end{table}
%%
\clearpage
  \begin{table}[hp]
\caption{TG + RCM (standalone)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
    arenas-jazz& 0.2899& 0.3079& 0.3206& 0.01& 13.0& 18.8333& 35.0& 3.9756

\\ \hline
arenas-meta &0.2335& 0.2753& 0.3129& 0.0234& 33.0& 43.1667& 58.0& 7.1698

\\ \hline
brunson & 0.3322& 0.4199& 0.431& 0.0229& 8.0& 9.8333& 13.0& 1.098

\\ \hline
contact &  0.0777& 0.0941& 0.108& 0.0094& 20.0& 27.4667& 39.0& 5.4328

\\ \hline
moreno\_oz &0.2605& 0.3139& 0.3388& 0.0236& 15.0& 26.6667& 50.0& 8.1459

 \\ \hline
 sociopatterns\_infectious&0.3872& 0.4262& 0.4633& 0.0224& 29.0& 39.9333& 60.0& 6.8844

\\
    \hline
  \end{tabular}
  \label{tab:TGRCMstandalone}
\end{table}
%%


  \begin{table}[hp]
\caption{TG + RCM + same part (standalone)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
    arenas-jazz& 0.2968& 0.3057& 0.3134& 0.0039& 12.0& 15.6667& 20.0& 2.1654

\\ \hline
arenas-meta &0.2467& 0.278& 0.3104& 0.0191& 31.0& 41.6333& 61.0& 6.57

\\ \hline
brunson & 0.3961& 0.4253& 0.431& 0.0118& 4.0& 6.0333& 11.0& 1.4256

\\ \hline
contact &  0.0801& 0.0989& 0.1092& 0.0086& 18.0& 25.2667& 35.0& 3.8465

\\ \hline
moreno\_oz &0.2589& 0.3286& 0.3388& 0.014& 16.0& 21.4667& 34.0& 4.3645

 \\ \hline
 sociopatterns\_infectious&0.416& 0.4531& 0.4633& 0.0118& 14.0& 20.4& 27.0& 2.8937

\\
    \hline
  \end{tabular}
\end{table}

%%


  \begin{table}[hp]
\caption{TG (DWave) (standalone)}
  \begin{tabular}{ |l|l|l|l|l|l|l|l|l|}
    \hline
    Graph & $Q_{\min}$ & $Q_{\mu}$ & $Q_{\max}$ &$std$& $it_{\min}$&$it_{\mu}$&$it_{\max}$& $std_{it}$\\ \hline
    arenas-jazz& 0.2897& 0.3091& 0.3204& 0.0094& 6.0& 9.9& 20.0& 2.7

\\ \hline
arenas-meta &0.2339& 0.2736& 0.3158& 0.0227& 9.0& 15.6& 35.0& 5.3827


\\ \hline
brunson & 0.3322& 0.4019& 0.431& 0.0335& 3.0& 4.5& 9.0& 1.3354


\\ \hline
contact &  0.0755& 0.0912& 0.1058& 0.0086& 7.0& 10.3667& 17.0& 2.7384


\\ \hline
moreno\_oz &0.258& 0.306& 0.3387& 0.0274& 6.0& 11.8667& 20.0& 3.3139


 \\ \hline
 sociopatterns\_infectious&0.3612& 0.4133& 0.4633& 0.0271& 9.0& 12.8& 18.0& 2.358


\\ \hline
  \end{tabular}
\end{table}
